How Transformers Utilize Multi-Head Attention in In-Context Learning? A Case Study on Sparse Linear Regression

Despite the remarkable success of transformer-based models in various real-world tasks, their underlying mechanisms remain poorly understood. Recent studies have suggested that transformers can implement gradient descent as an in-context learner for linear regression problems and have developed various theoretical analyses accordingly. However, these works mostly focus on the expressive power of transformers by designing specific parameter constructions, lacking a comprehensive understanding of their inherent working mechanisms post-training. In this study, we consider a sparse linear regression problem and investigate how a trained multi-head transformer performs in-context learning. We experimentally discover that the utilization of multi-heads exhibits different patterns across layers: multiple heads are utilized and essential in the first layer, while usually only a single head is sufficient for subsequent layers. We provide a theoretical explanation for this observation: the first layer preprocesses the context data, and the following layers execute simple optimization steps based on the preprocessed context. Moreover, we demonstrate that such a preprocess-then-optimize algorithm can significantly outperform naive gradient descent and ridge regression algorithms. Further experimental results support our explanations. Our findings offer insights into the benefits of multi-head attention and contribute to understanding the more intricate mechanisms hidden within trained transformers.

==> Sections/finding.tex <==
\section{Utilization of Multi-Head Attentions}

==> Sections/prelim.tex <==

\section{Preliminaries}\label{Sec:prelim}

\paragraph{Sparse Linear Regression.} We consider sparse linear models where $(\xb,y)\sim \mathsf{P}=\mathsf{P}^{\mathsf{lin}}_{\wb^\star}$ is sampled as $\xb\sim \mathsf{N}\paren{\boldsymbol{0}, \bSigma}$, $y=\la \wb^\star, \xb \ra+\mathsf{N}\paren{0, \sigma^2}$, where the  $\bSigma$ is a diagonal matrix and ground truth $\wb^\star\in \mathbb{R}^d$ satisfies $\|\wb^\star\|_0\leq s$. Then,  we  define the population risk of a parameter $\wb$ as follows: 
\begin{align*}
L(\wb):=\EE_{(\xb,y)\sim \mathsf{P}}\big[(\la \xb,\wb \ra-y)^2\big].
\end{align*}
Moreover, we are interested in the excess risk, i.e., the gap between the population risk achieved by $\wb$ and the optimal one:
\begin{align*}
\mathcal{E}(\wb):= L(\wb)-\min_{\wb} L(\wb).
\end{align*}

\paragraph{Multi-head Transformers.} Transformers are a type of neural network with stacked attention and multi-layer perceptron (MLP) blocks. In each layer, the transformer first utilizes multi-head attention $\mathsf{Attn}$ to process the input sequence (or hidden states) $\Hb = [\hb_{1}, \hb_{2}, \ldots, \hb_{m}] \in \mathbb{R}^{d_{\mathsf{hid}} \times m}$. It computes $h$ different queries, keys, and values, and then concatenates the output of each head:
\begin{align*}
    \mathsf{Attn}(\Hb,\mathbf{\theta_1}) = \Hb + \mathsf{Concat}[\Vb_1 \mathsf{sfmx}(\Kb_1^\top \Qb_1),\cdots,\Vb_h \mathsf{sfmx}(\Kb_h^\top \Qb_h)],
\end{align*}
% \in \RR^{\frac{d_{\mathsf{hidden}}}{h} \times n}
where $\Vb_i = \Wb_{V_i} \Hb,\Qb_i = \Wb_{Q_i} \Hb,\Vb_i = \Vb_{V_i} \Hb $ and $\mathbf{\theta_1} = \set{\Wb_{V_i},\Wb_{K_i},\Wb_{Q_i} \in \RR^{d_{\mathsf{hid}}/h \times d_{\mathsf{hid}}}}_{i=1}^{h}$ are learnable parameters. The $\mathsf{MLP}$ then applies a nonlinear element-wise operation:
\begin{align}\label{eq:MLP}
    \mathsf{MLP}(\Hb,\mathbf{\theta_2}) = \Wb_1 \mathsf{ReLU}(\Wb_2 \mathsf{Attn}(\Hb,\mathbf{\theta_1})),
\end{align}
where $\theta_2=\{\Wb_1,\Wb_2\}$ denotes the parameters of MLP. We remark that here some modules, such as layernorm and bias, are ignored for simplicity. 
% Note that the model parameters number is independent of the number of attention heads $h$, as each head projects the sequence into a $\frac{d_{\mathsf{hid}}}{h}$ subspace and then processes them.

\paragraph{Linear Attention-only Transformers} 
To perform an intractable theoretical investigation on the role of multi-head in the attention layer, we make further simplification on the transformer model by considering linear attention-only transformers. These simplifications are widely adopted in many recent works to study the behavior of transformer models \cite{vonoswaldTransformersLearnIncontext2023,zhang2023trained,mahankaliOneStepGradient2023,ahnTransformersLearnImplement}. In particular, the $i$-th layer $\mathsf{TF}_i$ performs the following update on the input sequence (or hidden state) $\Hb^{(i-1)}$ as follows:
\begin{align}\label{eq:lsa_mha}
    \Hb^{(i)} = \mathsf{TF}_i(\Hb^{(i-1)}) = \Wb_1 \big(\Hb^{(i-1)} + \mathsf{Concat}[\{\Vb_i \Mb \Kb_i^\top  \Qb_i \}_{i=1}^h]\big), \quad \Mb:= \begin{NiceArray}{\left\lgroup cc \right\rgroup}
\Ib_{n}& \mathbf{0}\\
\mathbf{0} & \mathbf{0}
\end{NiceArray} \in \RR^{m \times m},
\end{align}
where $\{\Wb_{V_i}, \Wb_{K_i}, \Wb_{Q_i} \in \RR^{\frac{d_{\mathsf{hid}}}{h} \times d_{\mathsf{hid}}}\}_{i=1}^{h}$ and $\Wb_1  \in \RR^{d_{\mathsf{hid}} \times d_{\mathsf{hid}}}$ are learnable parameters, note that as we ignore the $\mathsf{ReLU}$ activation in \Eqref{eq:MLP}, so we merge the parameter $\Wb_1 $ and $\Wb_2$ into one matrix $\Wb_1$. Besides, the mask matrix $\Mb$ is included in the attention to constrain the model focus the first $n$ in-context examples rather than the subsequent $m-n$ queries \cite{ahnTransformersLearnImplement,mahankaliOneStepGradient2023,zhang2024context}. To adapt the transformer for solving sparse linear regression problems, we introduce additional linear layers $\Wb_E \in \mathbb{R}^{(d+1) \times d_{\mathsf{hid}}}$ and $\Wb_{O} \in \mathbb{R}^{d_{\mathsf{hid}} \times 1}$ for input embedding and output projection, respectively. Mathematically, let $\Eb$ denotes the input sequences with $n$ in-context example followed by $q$ queries, 
\begin{align}\label{eq:tf_input}
\Eb = \begin{NiceArray}{\left\lgroup ccccccc \right\rgroup}
\xb_1 & \xb_2 & \cdots & \xb_{n}& \xb_{n+1}&\cdots &\xb_{n+q}\\
y_1 & y_2 & \cdots & y_{n}& 0&\cdots &0\\
\end{NiceArray}.
\end{align}
Then model processes the input sequence $\Eb$, resulting in the output $\hat{\yb} \in \RR^{1 \times (n+q)}$:
\begin{align*}
\hat{\yb} = \Wb_{O} \circ \mathsf{TF}_L \circ \cdots \circ \mathsf{TF}_1 \circ \Wb_{E} (\Eb),
\end{align*}

here, $L$ is the layer number of the transformer, and $\hat{y}_{i+n}$ is the prediction value for the query $\xb_{i+n}$. During training, we set $q > 1$ for efficiency, and for inference and theoretical analysis, we set $q = 1$ and define the in-context learning excess risk $\mathcal{E}_{\mathsf{ICL}}$ as:
\begin{align*}
\mathcal{E}_{\mathsf{ICL}} := \EE_{(\xb,y)\sim \mathsf{P}} (\hat{y}_{n+1} - y_{n+1})^2 - \sigma^2.
\end{align*}

\paragraph{Notations.}
For two functions $f(x) \geq 0$ and $g(x) \geq 0$ defined on the positive real numbers ($x > 0$), we write $f(x) \lesssim g(x)$ if there exists two constants $c,x_0 > 0$  such that $\forall x \geq x_0$, $f(x) \leq c \cdot g(x)$; we write $f(x) \gtrsim g(x)$ if $g(x) \lesssim f(x)$; we write $f(x) \backsimeq g(x)$ if $f(x) \lesssim g(x)$ and $g(x) \lesssim f(x)$. If $f(x) \lesssim g(x)$, we can write $f(x)$ as $O(g(x))$. We can also write write $f(x)$ as $\tilde{O}(g(x))$ if there exists a constant $k > 0$ such that $f(x) \lesssim g(x) \log^{k}(x)$.
% \section{A Possible Mechanism}\label{sec: Mechanism}
% Based on observations from our experiments on performing sparse linear regression with transformers, we found that each head in the first layer of the trained transformer is crucial, while in subsequent layers, only one head plays a significant role. Therefore, we hypothesize that the trained transformer implements data preprocessing in the first layer, whereas subsequent layers perform gradient descent on the least squares loss function. Next, we propose a date pre-processing algorithm which the trained transformer is likely to implement.


% \begin{algorithm*}[t]
% \caption{\DPPSlR}\label{alg:DPPSLR}
% \small
% \begin{algorithmic}[1]
%   \STATE \textbf{Input :} Data set $\set{(\xb_i,y_i)}_{i=1}^n$.
  
  
%   \FOR{k=1,\ldots, n} 
%   \STATE Compute $\tilde{\xb}_k$ by $\tilde{\xb}_k=\Rh\xb_k$, where 
% $\Rh=\mathsf{diag}\set{\hat{r}_1, \hat{r}_2, \ldots, \hat{r}_d}$,
%   where $\hat{r}_j$ is  given by
%   \begin{align}
%       \hat{r}_j=\frac{1}{n}\sum_{i=1}^n \xb_{ij}y_i,
%   \end{align}
%   where $\xb_{ij}$ is the $j$-th entry of $\xb_i$.
%   \ENDFOR
% \STATE \textbf{Output :} Data set $\set{\paren{\tilde{\xb}_i,y_i}}_{i=1}^n$
% \end{algorithmic}
% \end{algorithm*}
% \paragraph{Intuition for Algorithm~\ref{alg:DPPSLR}} ...




==> conclu.tex <==
%!TEX root =paper.tex


%\section{Conclusion} \label{sec:conclusion}

==> icml2024_TF2M/notations.tex <==
\def \parab{\overline{\para}}
\def \parab{\overline{\para}}
\newcommand{\rew}{\mathcal{R}^{\msf{all}}}
\newcommand{\rewfb}{\mathcal{R}^{\msf{feas}}_{[-B,B]}}
\newcommand{\rewfone}{\mathcal{R}^{\msf{feas}}_{[-1,1]}}
\newcommand{\rewfth}{\mathcal{R}^{\msf{feas}}_{[-3H,3H]}}

\newcommand{\tO}{\widetilde{\cO}}

\def \Vf{V^{\pp,r}}
\def \Qf{Q^{\pp,r}}
\def \piE{\pi^{\msf{E}}}
\def \hatpiE{\hat{\pi}^{\msf{E}}}
\def \pA{\overline{\cA}}
\def \pV{\overline{\cV}}
\def \para{\Theta}
% \def \rewm{\mathscr{R}}
% \def \RR{\rewm}
\def \fedb{e}
\def \wellpi{\Delta}
\def \wellsupp{n^{\msf{E}}}
\def \valsupp{n^{\msf{val}}}
\newcommand{\dpi}{d^\pi}
\newcommand{\dpiTheta}{d^\pi}
\newcommand{\DpiTheta}{D^\pi_\para}
\newcommand{\dall}{d^{\sf all}}
\newcommand{\dallTheta}{d^{{\sf all}}}
\newcommand{\DallTheta}{D^{\sf all}_\Theta}
\def \cn{\log\mathcal{N}(\Theta; \eps/H)}
\def \cns{\log\mathcal{N}}
\def \dimt{\dim\paren{\para}}
\def \pib{\pi^{\msf{b}}}
% \def \pival{\pi^{\msf{val}}}
\def \pival{\pi^{\msf{eval}}}
\def \dpival{d^{\pival}}
\def \Dpivalt{D^{\pival}_\Theta}
\def \DpiEt{D^{\piE}_\Theta}
% \def \hRR{\widehat{\RR}}
% \def \sRR{\RR^\star}
\def \hpp{\widehat{\pp}}
\def \DH{D^{\msf{H}}}
\def \DM{D^{\msf{M}}}
\def \Pidet{\Pi^{\mrm{determ}}}
\def \dpip{d^{\pp,\pi}}
\def \wellp{\eta}
\def \dt{\mrm{dim}\paren{\Theta}}
\def \hsa{[H]\times \cS\times \cA}


% Norms for convenience, along with sizes
% \newcommand{\norm}[1]{\left\|{#1}\right\|} % A norm with 1 argument
\newcommand{\lone}[1]{\norm{#1}_1} % l1 norm
\newcommand{\ltwo}[1]{\norm{#1}_2} % l2 norm
\newcommand{\lop}[1]{\norm{#1}_{\mathrm{op}}}
\newcommand{\lops}[1]{\|{#1}\|_{\mathrm{op}}}
\newcommand{\linf}[1]{\norm{#1}_\infty} % l-infinity norm
\newcommand{\lzero}[1]{\norm{#1}_0} % l0 norm
\newcommand{\dnorm}[1]{\norm{#1}_*} % Dual norm
\newcommand{\lfro}[1]{\left\|{#1}\right\|_{\sf Fr}} % Frobenius norm
\newcommand{\lnuc}[1]{\left\|{#1}\right\|_*} % Nuclear norm
\newcommand{\matrixnorm}[1]{\left|\!\left|\!\left|{#1}
  \right|\!\right|\!\right|} % Matrix norm with three bars
% \newcommand{\opnorm}[1]{\norm{#1}_{\rm op}} % Operator norm with three bars
\newcommand{\normbigg}[1]{\bigg\|{#1}\bigg\|} % A norm with 1 argument and bigg
                                              % brackets.
\newcommand{\normbig}[1]{\big\|{#1}\big\|} % A norm with 1 argument and big
                                           % brackets.
\newcommand{\normBig}[1]{\Big\|{#1}\Big\|} % A norm with 1 argument and Big
                                           % brackets
\newcommand{\lonebigg}[1]{\normbigg{#1}_1} % l1 norm
\newcommand{\ltwobigg}[1]{\normbigg{#1}_2} % l2 norm
\newcommand{\ltwobig}[1]{\normbig{#1}_2} % l2 norm
\newcommand{\ltwoBig}[1]{\normBig{#1}_2} % l2 norm
\newcommand{\linfbigg}[1]{\normbigg{#1}_\infty} % l-infinity norm
\newcommand{\norms}[1]{\|{#1}\|} % A norm with 1 argument and normal (small)
                                 % brackets.
\newcommand{\matrixnorms}[1]{|\!|\!|{#1}|\!|\!|} % Small matrix norm
\newcommand{\matrixnormbigg}[1]{\bigg|\!\bigg|\!\bigg|{#1}\bigg|\!\bigg|\!\bigg|} % Small matrix norm
\newcommand{\lones}[1]{\norms{#1}_1} % l1 norm with small brackets
\newcommand{\ltwos}[1]{\norms{#1}_2} % l2 norm with small brackets
\newcommand{\ltwob}[1]{\big\|#1\big\|_2}
\newcommand{\linfs}[1]{\norms{#1}_\infty} % l-infinity norm with small brackets
\newcommand{\lzeros}[1]{\norms{#1}_0} % l0 norm with small brackets
\newcommand{\lambdamax}[1]{\lambda_{\max}({#1})}
\newcommand{\lambdamin}[1]{\lambda_{\min}({#1})}
\newcommand{\vmax}[1]{v_{\max}({#1})}
\newcommand{\vmin}[1]{v_{\min}({#1})}


% Copied from headers of main text 
\def \dis{{d}}
% \def \cblue{\color{blue}}
% \def \cblack{\color{black}}
\def \cblue{}
\def \cblack{}
\newcommand{\online}{}
\newcommand{\bsh}{\textbackslash}
\newcommand{\va}{\V\times\a}
\def \dtheta{\mathrm{dim}\paren{\Theta}}
\def \Ctran{C^{\msf{tran}}}
\def \wCtran{C^{\msf{wtran}}}



% {\bf notations}
% \begin{itemize}
%  \item $\cA,~\cS,~ H$.~\yub{$\cA$ collides with $\cA$ set. Also, shall we use $\real^\cS$ or $\real^S$?}
% \item $r=\set{r_h(s,a)}_{h\in [H]},$
% \item $\pi=\set{\pi_h(\cdot|s)}_{h\in[H]}$
% \item $V^\pi_h(s;r,\pp)$. When it's clear from context, use $V^\pi_h(s;r)$.
% \item $Q^{\pi}_h(s, a;r)$
% \item \MDPR{}: $\m$. IRL problem: $\paren{\m, \piE}$.
% \item $d^\pi_h(s) \defeq \p(s_h = s|\pi)$
% \item $d^\pi_h(s, a) \defeq\p(s_h = s, a_h = a|\pi)$
% \item $A^{\pi}_h(s,a)$
% \item $\m\cup r$
% \item \textbf{operator.} $\brac{\pp_h V_{h+1}}(s,a)$, $\brac{\v_h V_{h+1}}(s,a)$, $\widehat{\pp}_h$, $\widehat{\v}_h$
% \item \textbf{feasible reward set.} $\cR_{\m,\piE}$
% \item \textbf{parameter set:} $A\in \pA$, $V\in \pV$. $\theta=(A,V)\in \para$~\yub{to be changed}
% \item \textbf{reward mapping:} $\rewm$, $r^\theta=\rewm\paren{V,A}=\rewm\paren{\theta}$
% \item \textbf{Feadback.} $\fedb$.
% \item \textbf{well-posedness.} for $\supp$: $\wellsupp$, for $\piE_h(a|s)$: $\wellpi$.
% \item \textbf{dimension of parameter space:} $\dimt$
% \item  \textbf{behavior policy:} $\pib$, \textbf{evaluation policy:} $\pival$, $\dpival$
% \item \textbf{metric for rewards.} $\dallTheta$, $\dpiTheta$, $\dpival$.
% \item \textbf{metric for reward mappings.} $\DallTheta$, $\DpiTheta$, $\Dpivalt$.
% \item \textbf{set of rewards.} $\rew$.
% \item \textbf{ground truth reward mapping.} $\sRR$, \textbf{recovered reward mapping.} $\hRR$.
% \item \textbf{recovered dynamics.} $\hpp$.
% \item \textbf{Hausdorff metric.} $\DH$. Mapping-based metric: $\DM$.
% \item \textbf{optimal policy set.} $\Pi^\star_{\m\cup r}$
% \end{itemize}




\def \DPPSlR{\textsc{Data Pre-processing for Sparse Linear Regression}}
\def \P{\mathsf{P}}
\def \wt{{\hat{\wb}_t}}
\def \ws{{\wb^\star}}
\def \Sigmab{\mathbf{\Sigma}}
\def\Xt{\tilde{\Xb}}
\def \xt{\tilde{\xb}}
\def \Sigmah{\hat{\Sigmab}}
\def \Sigmal{\overline{\Sigmab}}
\def\epsb{\mathbf{\epsilon}}
\def \Sigmat{\tilde{\Sigmab}}
\def \Rh{\hat{\Rb}}
\def \zerob{\mathbf{0}}
\def \contt{\alpha}
\def \nn{\frac{1}{n}}
\def \nnn{\frac{1}{n^2}}
\def \EEE{\cE}
\def \cont{{\tilde{\alpha}}}
\def \At{\tilde{\Ab}}
\def \wts{\tilde{\wb}^\star}
\def \Rl{\overline{\Rb}}
\def \whp{with probability at least $1-\delta$}
\def \wla{\hat{\wb}_{\lambda}}
\def\XXb{\Xb\Xb^\top}
\def\wols{\wb_{\mathrm{ols}}}
\def \wpre{{\hat{\wb}}}
\def \wgd{\wb_{\mathsf{gd}}}
\def \twgd{\tilde{\wb}_{\mathsf{gd}}}

==> icml_sections/abstract.tex <==
\begin{abstract}

% Despite the remarkable success of transformer-based models in various real-world tasks, the theoretical understanding of their mechanisms remains limited. Recent works have explored the in-context learning ability of transformers, but proposed key mechanisms often lack experimental validation. In this study, we investigate the role of multi-head attention in transformers for in-context learning using the sparse linear regression problem as a testbed. Through our experiments, we discovered that multiple heads are essential in the first layer, whereas single heads are usually sufficient for subsequent layers. Supported by additional experiments, we propose a framework in which the first layer preprocesses the data, and the following layers perform simple optimization steps based on the preprocessed context. We offer theoretical explanations of how transformers leverage this algorithm to outperform gradient descent and ordinary least squares/ridge regression. Furthermore, we demonstrate the effectiveness of our proposed algorithm under more complex data distributions. Our findings provide valuable insights into the benefits of multi-head attention and contribute to a deeper understanding of the intricate mechanisms within trained transformers.
% -- revised --
% Despite the remarkable success of transformer-based models in various real-world tasks, their underlying mechanisms remain poorly understood. Recent studies have suggested that transformers can implement gradient descent as an in-context learner for linear regression problems and have developed various theoretical analyses accordingly. However, these works mostly focus on the expressive power of transformers by designing specific parameter constructions, lacking a comprehensive understanding of their inherent working mechanisms post-training. In this study, we consider a sparse linear regression problem and investigate how a trained multi-head transformer performs in-context learning. We experimentally discover that the utilization of multi-heads exhibits different patterns across layers: multiple heads are utilized and essential in the first layer, while usually one single head is dominantly utilized for subsequent layers. We provide a theoretical rationale for this observation: the first layer undertakes data preprocessing on the context examples, and the following layers execute simple optimization steps based on the preprocessed context. Moreover, we prove that such a preprocess-then-optimize algorithm can outperform naive gradient descent and ridge regression algorithms, which is also supported by our further experiments. Our findings offer insights into the benefits of multi-head attention and contribute to understanding the more intricate mechanisms hidden within trained transformers.

% Despite the remarkable success of transformer-based models in various real-world tasks, their underlying mechanisms remain poorly understood. Recent studies suggest transformers can implement gradient descent for linear regression and developes various theoretical analyses accordingly, but mainly focus of these work is on expressive power through specific parameter constructions, lacking insights into their working mechanisms post-training. 
In this study, we investigate how a trained multi-head transformer performs in-context learning on sparse linear regression. We experimentally discover distinct patterns in multi-head utilization across layers: multiple heads are essential in the first layer, while subsequent layers predominantly utilize a single head. We propose that the first layer preprocesses input data, while later layers execute simple optimization steps on the preprocessed data. Theoretically, we prove such a preprocess-then-optimize algorithm can outperform naive gradient descent and ridge regression, corroborated by experiments. Our findings provide insights into the benefits of multi-head attention and the intricate mechanisms within trained transformers.

% We first design a new IRL algorithm for the offline setting, Reward Learning with Pessimism (RLP), and show that it achieves polynomial sample complexity in terms of the size of the MDP, a concentrability coefficient between the behavior policy and the expert policy, and the desired accuracy. Building on RLP, we further design an algorithm Reward Learning with Exploration (RLE), which operates in a natural online setting where the learner can both actively explore the environment and query the expert policy, and obtain a stronger notion of IRL guarantee from polynomial samples. We establish sample complexity lower bounds for both settings showing that RLP and RLE are nearly optimal. Finally, as an application, we show that the learned reward functions can \emph{transfer} to another target MDP with suitable guarantees when the target MDP satisfies certain similarity assumptions with the original (source) MDP. \yub{shorten}

\end{abstract}


% ICLR/arxiv version
% Inverse Reinforcement Learning (IRL)---the problem of learning reward functions from demonstrations of an \emph{expert policy}---plays a critical role in developing intelligent systems, such as those that understand and imitate human behavior. While widely used in applications, theoretical understandings of IRL admit unique challenges and remain less developed compared with standard RL theory. For example, it remains open how to do IRL efficiently in standard \emph{offline} settings with pre-collected data, where states are obtained from a \emph{behavior policy} (which could be the expert policy itself), and actions are sampled from the expert policy.
% This paper provides the first line of results for efficient IRL in vanilla offline and online settings using polynomial samples and runtime. We first design a new IRL algorithm for the offline setting, Reward Learning with Pessimism (RLP), and show that it achieves polynomial sample complexity in terms of the size of the MDP, a concentrability coefficient between the behavior policy and the expert policy, and the desired accuracy. Building on RLP, we further design an algorithm Reward Learning with Exploration (RLE), which operates in a natural online setting where the learner can both actively explore the environment and query the expert policy, and obtain a stronger notion of IRL guarantee from polynomial samples. We establish sample complexity lower bounds for both settings showing that RLP and RLE are nearly optimal. Finally, as an application, we show that the learned reward functions can \emph{transfer} to another target MDP with suitable guarantees when the target MDP satisfies certain similarity assumptions with the original (source) MDP. \yub{shorten}

==> icml_sections/conclu.tex <==
%!TEX root =paper.tex

\vspace{-.5em}
\section{Conclusions}
\label{sec:conclusion}
% \vspace{-.5em}

In this paper, we investigate a sparse linear regression problem and explore how a trained transformer leverages multi-head attention for in-context learning. Based on the experiment and theoretical characterizations, we show that transformer may implement the preprocess-then-optimize algorithm, by using multiple heads in the first layer and one head in the subsequent layer. Numerical experiments support our findings.


% Based on our empirical investigations, we propose a preprocess-then-optimize algorithm, where the trained transformer utilizes multi-head attention in the first layer for data preprocessing, and subsequent layers employ only a single head for optimization. We theoretically prove the effectiveness of our algorithm compared to OLS, ridge regression, and gradient descent, and provide additional experiments to support our findings. 

% While our findings provide promising insights into the hidden mechanisms of multi-head attention for in-context learning, there is still much to be explored. First, our work focuses on the case of sparse linear regression, and it may be beneficial to implement our experiment for more challenging or even real-world tasks. Additionally, as we adapt attention-only transformers for analysis simplification, the role of other modules, such as MLPs, are neglected. How these modules incorporate in real-world tasks remains unclear. Moreover, our analysis does not consider the training dynamics of transformers, how transformers learn to implement these algorithms is worth further investigation.

% In this paper, we propose a novel algorithm for Inverse Reinforcement Learning (IRL) in the offline setting, using polynomial samples and runtime. Building upon our offline algorithm, we design an algorithm for IRL in the online setting, employing the same complexity as prior work, but under a stronger performance metric. We believe our work opens up many important questions, such as designing better metrics for IRL problems, generalizing our IRL algorithms to the function approximation setting, and developing more computationally efficient algorithms.

==> icml_sections/exp_insight.tex <==
\section{Experimental Insights into Multi-head Attention for In-context Learning}\label{sec:exp_insight}

\begin{figure*}[!t]
\vspace{-.1in}
  \centering
\begin{subfigure}{0.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{pic/setting.pdf}
  % \caption{Overview of the experiments, including task, data, architecture, and our insights.}
  \caption{}
  \label{fig:sfig1}
\end{subfigure}
\begin{subfigure}{.175\textwidth}
  \centering
  \includegraphics[width=\linewidth]{pic/exp/bert/risk_comp_4_4_0.1.pdf}
  % \caption{Varying Heads}
  \caption{}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.165\textwidth}
  \centering
  \includegraphics[width=\linewidth]{pic/exp/bert/mask_head_4_4.pdf}
  % \caption{Heads Assessment}
  \caption{}
  \label{fig:sfig3}
\end{subfigure}
\begin{subfigure}{.175\textwidth}
  \centering
  \includegraphics[width=\linewidth]{pic/exp/bert/prob_4_4_0.1.pdf}
  % \caption{Pruning and Probing}
  \caption{}
  \label{fig:sfig4}
\end{subfigure}
\vskip -.1in
\caption{Experimental insights into multi-head attention for in-context learning. \textit{(a)}: Overview of the experiments, including task, data, architecture, and our insights. \textit{(b)}: ICL with Varying Heads. \textit{(c)}: Heads Assessment. \textit{(d)}: Pruning and Probing.}
\label{fig:overview}
% \vspace{-1em}
\end{figure*}

% While previous work has demonstrated the in-context learning ability for sparse linear regression \cite{gargWhatCanTransformers2023,baiTransformersStatisticiansProvable2023}, the hidden mechanism behind the trained transformer for solving this problem remains unclear. To this end, we design a series of experiments, utilizing techniques like probing \cite{alain2016understanding} and pruning\cite{li2017pruning} to help us gain initial insights into how the trained transformer utilizes multi-head attention for this problem. For all experiments in Sections \ref{sec:exp_insight} and \ref{sec:exp}, we choose an encoder-based architecture as the backbone (see \autoref{fig:sfig1}), set the hidden dimension $d_{\mathsf{hid}}$ to 256, and use the input sequence format shown in \Eqref{eq:tf_input}, where $d = 16$, $s = 4$, $\xb\sim \mathsf{N}\paren{\boldsymbol{0}, \Ib}$, with varying noise levels, layers, and heads, Additional experimental details can be found in Appendix~\ref{sec:exp_detail}. The experiments we designed are as follows:

% While previous work has demonstrated the in-context learning ability for sparse linear regression \cite{gargWhatCanTransformers2023,baiTransformersStatisticiansProvable2023}, the hidden mechanism behind the trained transformer for solving this problem remains unclear. Here, 

To understand the hidden mechanism behind the trained transformer, we design a series of experiments, utilizing techniques like probing \cite{alain2016understanding} and pruning\cite{li2017pruning} to help us gain initial insights into how the trained transformer utilizes multi-head attention. 

% For all experiments in Sections \ref{sec:exp_insight} and \ref{sec:exp}, we choose an encoder-based architecture as the backbone (see \autoref{fig:sfig1}), set $d_{\mathsf{hid}}=256$, $d = 16$, $s = 4$, experimental details can be found in Appendix~\ref{sec:exp_detail}. The experiments we designed are as follows:

\noindent\textbf{ICL with Varying Heads:} This experiment investigates the performance of transformers in solving in-context sparse linear regression with different numbers of attention heads. An example can be found in \autoref{fig:sfig2}, where we display the excess risk for different models when using different numbers of in-context examples. We can observe that given few-shot in-context examples, transformers can outperform OLS and ridge. Moreover, we can also clearly observe the benefit of using multiple heads, which leads to lower excess risk when increasing the number of heads. This \textbf{highlights the importance of multi-head attention in  transformer to perform in-context learning}.

\noindent\textbf{Heads Assessment:} This experiment evaluates the importance of each attention head by masking individual heads and measuring the change in risk.
% Based on \Eqref{eq:lsa_mha}, we know that the $j$-th head at the $i$-th layer corresponds to the subspace of the intermediate output from $(j-1) \cdot d_{\mathsf{hid}} / h$ to $ j \cdot d_{\mathsf{hid}} / h -1$. To assess the importance of each attention head, we can mask the particular head by zeroing out the corresponding output entries, while keeping other dimensions unchanged. Then, let $(i,j)$ be the layer and head indices, we evaluate the risk change before and after head masking, denoted by $\Delta \mathcal{E}_{\mathsf{ICL} (i,j)}$. Then we normalize the risk changes in the same layer to evaluate their relative importance:
% \begin{align}
% \mathcal{W}_{i,j} = \frac{\Delta \mathcal{E}_{\mathsf{ICL} (i,j)}}{\sum_{k = 1}^{h} \Delta \mathcal{E}_{\mathsf{ICL} (i,k)}}.
% \end{align}
An example can be found in \autoref{fig:sfig3}. We find that in the first layer, no head distinctly outweighs the others, while in the subsequent layers, there always exists a head that exhibits higher importance than others. This gives us insight that \textbf{in the first attention layer, all heads appear to be significant, while in the subsequent layers, only one head appears to be significant}.

\noindent\textbf{Pruning and Probing:} Based on the previous findings, this experiment prunes the trained model by retaining all heads in the first layer and only keeping the most important head in subsequent layers. The pruned model is then fine-tuned. Linear probes are used to evaluate the prediction performance of different layers.  An example can be found in \autoref{fig:sfig4}, it shows that the pruned model performs similarly to the original model, but differently from a single-head transformer. Noting that the main difference between them is the number of heads in the first layer (subsequent layers have the same structure),  it can be deduced that \textbf{the working mechanisms of the multi-head transformer may be different for the first and subsequent layers}.
% we can find that the ``pruned transformer'' and the original model exhibit almost the same performance for each layer. Additionally, compared to the model with single-head attention, we observe that the probing result is largely different between single-head transformers and the ``pruned transformers'', the latter has better performances compared to the former. Noting that the main difference between them is the number of heads in the first layer (subsequent layers have the same structure),  it can be deduced that \textbf{the working mechanisms of the multi-head transformer may be different for the first and subsequent layers}.


==> icml_sections/experiment.tex <==
\vspace{-.05in}
\section{Experiments}\label{sec:exp}
\vspace{-.05in}

In Section~\ref{sec:exp_insight}, we conduct several experiments, and based on the observations, we propose that a trained transformer can apply a preprocess-then-optimize algorithm. While the second part (gradient descent over context) is supported by extensive theoretical analysis and experimental evidence \citep{vonoswaldTransformersLearnIncontext2023,cheng2023transformers,zhang2023trained,ahnTransformersLearnImplement}, here we develop a technique called preprocessing probing (P-probing) on the trained transformer to support the first part of our algorithm, where we try to extract the preprocessed component $\set{\tilde{\xb}_i}_{i=n+1}^{n+q}$ from the first layer of transformer as in, as illustrated in \autoref{fig:exp_fig1}. We also directly apply Alg.~\ref{alg:DPPSLR} on the in-context examples and then check the excess risk for multiple-step gradient descent to verify the effectiveness of our algorithm and theoretical analysis. Experimental details can be found in Appendix~\ref{sec:exp_detail}.






Based on \autoref{fig:exp_fig2}, we can observe that compared to the transformer with single-head attention ($h=1$), the query entries extracted from the transformer with multiple heads ($h = 4,8$) preserve better convergence performance and can dive into a lower risk. This aligns well with our experiment result in \autoref{fig:exp_fig3}, where compared to \texttt{gd}, the data preprocessed by Alg.~\ref{alg:DPPSLR} preserves better convergence performance and can dive into a lower risk space, supporting the existence of the preprocessing procedure in the trained transformer. Moreover, \autoref{fig:exp_fig3} also aligns well with our theoretical analysis, where our algorithm can outperform ridge regression and OLS.

==> icml_sections/finding.tex <==
\section{Utilization of Multi-Head Attentions}

==> icml_sections/intro.tex <==

\section{Introduction}\label{sec:inro}

Transformers\cite{vaswaniAttentionAllYou2023} have shown remarkable performance in natural language processing \cite{ouyang2022training,achiam2023gpt,brown2020language,radford2019language} and other domains \cite{dosovitskiy2020image,peebles2023scalable}, exhibiting capabilities like in-context learning\cite{brown2020language,xie2021explanation}. While numerous studies have explored transformers' expressive power\cite{kajitsukaAreTransformersOne2023,takakuraApproximationEstimationAbility2023} and ability to emulate algorithms\cite{guoHowTransformersLearn2023,baiTransformersStatisticiansProvable2023,liTransformersAlgorithmsGeneralization,chen2024can}, understanding their inner workings remains a challenge, especially the roles of different attention layers and heads.

This work investigates how transformers utilize multi-head attention across layers for in-context learning on sparse linear regression tasks. Empirically, we observed a distinct pattern: while the first attention layer utilized all heads evenly, subsequent layers predominantly relied on a single head. This suggests different working mechanisms for the first and later layers. Based on these findings, we propose that transformers employ a preprocess-then-optimize algorithm: the first layer preprocesses input data using multiple heads, then subsequent layers perform iterative optimization (e.g., gradient descent) on the preprocessed data using a single head. We theoretically demonstrate that such an algorithm can be implemented by a modestly-sized transformer and achieve lower excess risk than traditional methods like gradient descent and ridge regression without preprocessing.

Our main contributions are: 
\begin{itemize}[leftmargin=*,nosep]
\item We empirically revealing the distinct head utilization patterns across layers.
\item Building upon our empirical findings, we proposed a possible working mechanism for multi-head transformers. 
\item We further validated our proposed mechanism by theoretical analysis.
\item We conducted additional experiments to further validate our theoretical framework.
\end{itemize}
% 1) Empirically revealing the distinct head utilization patterns across layers; 2) Proposing the preprocess-then-optimize mechanism and theoretically validating its implementability; 3) Proving and experimentally verifying the excess risk advantage of this mechanism over traditional methods; 4) Further empirical support through probing experiments on the first layer's output representations.




==> icml_sections/mechanism.tex <==
\section{Potential Mechanism Behind Trained transformer}\label{sec:Mechanism}
% Based on the experimental insights from Section \ref{sec:exp_insight}, we found that all heads in the first layer of the trained transformer are crucial, while in subsequent layers, only one head plays a significant role. Furthermore, by checking the result for probing and pruning, we can find that the working mechanisms of the transformer may be different for the first and subsequent layers. To this end, we hypothesize that the multi-layer transformer may implement a preprocess-then-optimize to perform the in-context learning, i.e., the transformer first performs preprocessing on the in-context examples using the first layer and then implements multi-step iterative optimization algorithms on the preprocessed in-context examples using the subsequent layers. 

Based on the experimental insights from Section \ref{sec:exp_insight}, we found that while all heads in the first layer are crucial, only one head plays a significant role in subsequent layers. Additionally, probing and pruning results suggest different working mechanisms for the first and subsequent layers. To this end, we hypothesize that the multi-layer transformer implements a preprocess-then-optimize approach for in-context learning, where the first layer preprocesses the in-context examples, and subsequent layers implement iterative optimization algorithms on the preprocessed data.
% We note that \cite{guoHowTransformersLearn2023} adapts a similar two-phase idea to explain how transformer learning specific functions in context, in their constructed transformers, the first few layers utilize MLPs to compute an appropriate representation for each entry, while the subsequent layers utilize the attention module to implement gradient descent over the context. We highlight that our algorithm mainly focus on utilizing multihead attention model, and it aligns well with the our experimental observation and intuition. The details of our algorithm are as follows:

% \dz{perhaps mention that the first part is similar to the feature learning mechanism in Mei song's paper and the second part is general in many recent icl paper?}

% hypothesize that \textit{the trained transformer tends to implement data preprocessing in the first layer with multihead attention, whereas subsequent layers perform gradient descent on the least squares loss function}. \dz{need to mention existing works on the connection between single-head attention layer and one-step gradient descent}

% We abstract this preprocess-then-optimize algorithm for linear attention-only transformer to explain how can transformer implement this algorithm and then provide theoretical analysis to proof the effectiveness for this algorithm in \autoref{sec:main_theory}.

\subsection{Preprocessing on In-context Examples}

As the multihead attention is designed to facilitate to model to capture features from different representation subspaces \cite{vaswaniAttentionAllYou2023}, we abstract the algorithm implementation by the first layer of the transformers as a preprocessing procedure. In general, for the sparse linear regression, a possible data preprocessing method is to perform reweighting of the data features by emphasizing the features that correspond to the nonzero entries of the ground truth $\wb^*$ and disregard the remaining features. In the idealized case, if we know the nonzero support of $\wb^*$, we can trivially zero out the date features of $\xb$ on the complement of the nonzero support, as a data preprocessing procedure, and perform projected gradient descent to obtain the optimal solution. Although the nonzero support of $\wb^*$ is intractable to the learner, we can estimate each dimension $w_i^*$ by $\frac{1}{n}\sum_{i=1}^n x_{ij}y_i$, as $\EE[x_iy] = \EE[\sum_{i=1}^dw_i^*x_i\cdot x_i]+\EE[\xi x_i] = w_i^* \EE[x_i^2]$, resulting in Alg.~\ref{alg:DPPSLR}.



% In general, the nonzero support of $\wb^*$ is intractable to the learner, so that one cannot perform idealized masking-related data preprocessing. However, one can still perform estimations on the importance of data features by examining their correlation with the target. In particular, note that we have $
% y = \la\wb^*,\xb\ra +\xi_i = \sum_{i=1}^d w^*_ix_i + \xi_i$, implying that $r_i:=\EE[x_iy] = \EE[\sum_{i=1}^dw_i^*x_i\cdot x_i]+\EE[\xi x_i] = w_i^* \EE[x_i^2]$ if considering independent data features. Then it is clear that such a correlation between the feature and label will be nonzero only when $|w^*_i|\neq 0$. Therefore, instead of knowing the nonzero support of $\wb^*$, we can instead calculate such a correlation to perform reweighting on the data features. Noting that the transformer is provided with $n$ in-context examples $\set{(\xb_i,y_i)}_{i=1}^n$, such correlations can be estimated accordingly: $\hat r_j= \frac{1}{n}\sum_{i=1}^nx_{ij}y_i$, which will be further used to perform the data preprocessing on the in-context examples. We summarize this procedure  in Alg.~\ref{alg:DPPSLR}.

% The preprocessing procedure aligns well with the structure of a multi-head attention layer with linear attention, which motivates our theoretical construction of the desired transformer. In particular, each head of the attention layer can be conceptualized as executing specific operations on a distinct subset of data entries. Then, the linear query-key calculation, represented as $(\mathbf{W}_{K_i}\mathbf{H})^\top\mathbf{W}_{Q_i}\mathbf{H}$, where $\mathbf{H}=\mathbf{E}$ denotes the input sequence embedding matrix, effectively estimates correlations between the $i$-th subset of data entries and the corresponding label $y_i$. Here, $\mathbf{W}_{K_i}$ and $\mathbf{W}_{Q_i}$ selectively extract entries from the $i$-th subset of features and the label, respectively, akin to an "entries selection" process. Furthermore, when combined with the value calculation $\Wb_{V_i}\Hb$, each head of the attention layer conducts correlation calculations for the $i$-th subset of features and subsequently employs them to reweight the original features within the same subset. Consequently, by stacking the outputs of multiple heads, all data features can be reweighted accordingly, which matches the design of the proposed proprocessing procedure in Alg.~\ref{alg:DPPSLR}. We formally prove this in the following theorem.






% Note that $\EE_{(\xb,y)\sim \mathsf{P}} [\hat{r}_j | \wb^\star] = \wb^\star_j $, where $\wb^\star$ is a sparse parameter where the no-zero data is the desired sparse feature, so in this way we can keep the no related feature be small enough while keep the desired sparse feature still maintain the original magnitude. Moreover we can proof that there exists a single layer transformer with multi-head attention that can implement Algorithm~\ref{alg:DPPSLR}, resulting the following proposition:



% \begin{proposition}[Single-layer multi-head transformer implements Alg.~\ref{alg:DPPSLR}]\label{prop:pre-process}
% There exists a single-layer transformer function $\mathsf{TF}_1$, with $d$ heads and $d_{\mathsf{hid}} = 3d$  hidden dimension, together with an input embedding layer with weight $\Wb_E\in\RR^{d_{\mathsf{hid}}\times d}$, that can implement Alg.~\ref{alg:DPPSLR}.
% % and the input projection $\Wb_{E} \in \RR^{(d+1) \times d_{\mathsf{hid}}}$ 
% % such that the first attention layer can implement Algorithm \ref{alg:DPPSLR}. 
% Let $\Eb$ be the input sequence defined in \Eqref{eq:tf_input} and  $\tilde \xb_i = \hat\Rb\xb$ be the preprocessed features defined in Alg.~\ref{alg:DPPSLR}, it holds that% so that each of the enhanced data $\{\hat{r}_i \xb_{i,j}\}_{i \in [d]}$ can be found in the output representation $\Hb^{(1)}$:
% \begin{align}\label{eq:tf_h1}
% \Hb^{(1)} := \mathsf{TF}_1 \circ \Wb_{E}(\Eb) = \begin{NiceArray}{\left\lgroup ccccccc \right\rgroup }
% \tilde{\xb}_1 & \tilde{\xb}_2 & \cdots & \tilde{\xb}_{n}& \tilde{\xb}_{n+1}&\cdots & \tilde{\xb}_{n+q}\\
% y_1 & y_2 & \cdots & y_{n}& 0&\cdots&0\\
% \vdots&\vdots&\ddots&\vdots&\vdots&\ddots&\vdots\\
% \end{NiceArray},
% \end{align}
% where $\cdots$ in third row implies arbitrary values.
% \end{proposition}






\subsection{Optimizing Over Preprocessed In-Context Examples}

Based on the experimental results, we observe that the subsequent layers of transformers dominantly rely on one single head, suggesting their different but potentially simpler behavior compared to the first one. Motivated by a series of recent work \citep{vonoswaldTransformersLearnIncontext2023,cheng2023transformers,zhang2023trained} that reveal the connection between gradient descent steps and multi-layer single-head transformer in the in-context learning tasks, we conjecture that the subsequent layers also implement iterative optimization algorithms, e.g., gradient descent algorithm, on the (preprocessed) in-context examples. 


% To maintain clarity in our construction and explanation, in each layer, we use a linear projection $\Wb_1^{(i)}$ to rearrange the dimensions of the sequence processed by the multi-head attention, resulting in the hidden state $\Hb^{(i)}$ of each layer.  We refer to the first $d$ rows of the input data as $\xb$, and the $(d+1)$-th row as the corresponding $y$. For example, in \Eqref{eq:tf_h1}, we take the first $d$ rows, together with the $(d+1)$-th row, as the input data entry $\{ \tilde{\xb}_i, y_i \}_{i=1}^{n+1}$. Then, the following proposition shows that the subsequent layers of transformer can implement multi-step gradient descent on the preprocessed in-context examples $\{(\tilde \xb_i, y_i)\}_{i=1,\dots,n}$.
% \begin{proposition}[Subsequent single-head transformer implements multi-step GD]\label{prop:tf_gd}
% There exists a transformer with $k$ layers, $1$ head, $d_{\mathsf{hid}} = 3d$, let $\hat y_{n+1}^{\ell}$ be the  prediction representation of the $\ell$-th layer, then 
% % $\{(\tilde{\xb}_{i}, \hat{y}_{(i)}^{\ell})\}_{i = 1}^{n+1}$ be the $\ell$-th layer input data entry, 
% it holds that $\hat{y}_{(n+1)}^{\ell} =\la \wb_{\mathsf{gd}}^{\ell}, \tilde{\xb}_{n+1} \ra$, where $\tilde \xb_{n+1}=\hat \Rb\xb_{n+1}$ denotes the preprocessed data feature,  $\wb_{\mathsf{gd}}^\ell$ is defined as $\wb_{\mathsf{gd}}^{0} = 0$ and as follows for $\ell=0,\dots,k-1$:
% \begin{align}
%     \wb_{\mathsf{gd}}^{\ell +1} = \wb_{\mathsf{gd}}^{\ell} - \eta \nabla \tilde L(\wb_{\mathsf{gd}}^{\ell}),\quad \text{where} \quad \tilde L(\wb) = \frac{1}{2n} \sum_{i=1}^n (
%     y_i - \la \wb, \tilde{\xb}_{i} \ra)^2.
% \end{align}
% \end{proposition}

% The proof of Propositions \ref{prop:pre-process} and \ref{prop:tf_gd} can be found in Appendix~\ref{sec:proof_props}, combining these two propositions , we show that the multi-layer transformer with multiple heads in the first layer and one head in the subsequent layers can implement the proposed preprocess-then-optimization algorithm. In the next section, we will establish theories to demonstrate that such an algorithm can indeed achieve smaller excess risk than standard gradient descent and ridge regression solutions of the sparse linear regression problem.

We further prove that these two procedures (preprocessing then optimizing) can be implemented by linear attention-only transformers in Propositions \ref{prop:pre-process} and \ref{prop:tf_gd} (presented in Appendix). More details about our preprocess-then-optimize algorithm can be found in Appendix~\ref{sec:proof_props}.


\begin{figure}[t]
\vspace{-1em}
\begin{algorithm}[H]
\caption{Data preprocessing for in-context examples}\label{alg:DPPSLR}
\small
\begin{algorithmic}[1]
  \STATE \textbf{Input :} Sequence with $\set{(\xb_i,y_i)}_{i=1}^n, \set{(\xb_i,0)}_{i=n+1}^{n+q}$ as in-context examples/queries.
  \FOR{$k=1,\ldots, n$} 
  \STATE Compute $\tilde{\xb}_k$ by $\tilde{\xb}_k=\Rh\xb_k$,\\
  where 
$\Rh=\mathsf{diag}\set{\hat{r}_1, \hat{r}_2, \ldots, \hat{r}_d}$,
  where $\hat{r}_j$ is  given by
  \begin{align}
      \hat{r}_j=\frac{1}{n}\sum_{i=1}^n x_{ij}y_i.
  \end{align}
  \ENDFOR
\STATE \textbf{Output :} Sequence with the preprocessed in-context examples/queries $\set{\paren{\tilde{\xb}_i,y_i}}_{i=1}^n,\set{(\tilde{\xb}_i,0)}_{i=n+1}^{n+q}$ .
\end{algorithmic}
\end{algorithm}
% \vspace{-3em}
\end{figure}

==> icml_sections/prelim.tex <==

\section{Preliminaries}\label{Sec:prelim}

\paragraph{Sparse Linear Regression.} We consider sparse linear models where $(\xb,y)\sim \mathsf{P}=\mathsf{P}^{\mathsf{lin}}_{\wb^\star}$ is sampled as $\xb\sim \mathsf{N}\paren{\boldsymbol{0}, \bSigma}$, $y=\la \wb^\star, \xb \ra+\mathsf{N}\paren{0, \sigma^2}$, where the  $\bSigma$ is a diagonal matrix and ground truth $\wb^\star\in \mathbb{R}^d$ satisfies $\|\wb^\star\|_0\leq s$. Then,  we  define the population risk of a parameter $\wb$ as: 
\begin{align*}
L(\wb):=\EE_{(\xb,y)\sim \mathsf{P}}\big[(\la \xb,\wb \ra-y)^2\big].
\end{align*}
Moreover, we are interested in the excess risk:
\begin{align*}
\mathcal{E}(\wb):= L(\wb)-\min_{\wb} L(\wb).
\end{align*}

% \paragraph{Multi-head Transformers.} Transformers are a type of neural network with stacked attention and multi-layer perceptron (MLP) blocks. In each layer, the transformer first utilizes multi-head attention $\mathsf{Attn}$ to process the input sequence (or hidden states) $\Hb = [\hb_{1}, \hb_{2}, \ldots, \hb_{m}] \in \mathbb{R}^{d_{\mathsf{hid}} \times m}$. It computes $h$ different queries, keys, and values, and then concatenates the output of each head:
% \begin{align*}
%     \mathsf{Attn}(\Hb,\mathbf{\theta_1}) = \Hb + \mathsf{Concat}[\set{\Vb_i \mathsf{sfmx}(\Kb_i^\top \Qb_i)}_{i=1}^h],
% \end{align*}
% % \in \RR^{\frac{d_{\mathsf{hidden}}}{h} \times n}
% where $\Vb_i = \Wb_{V_i} \Hb,\Qb_i = \Wb_{Q_i} \Hb,\Vb_i = \Vb_{V_i} \Hb $ and $\mathbf{\theta_1} = \set{\Wb_{V_i},\Wb_{K_i},\Wb_{Q_i} \in \RR^{d_{\mathsf{hid}}/h \times d_{\mathsf{hid}}}}_{i=1}^{h}$ are learnable parameters. The $\mathsf{MLP}$ then applies a nonlinear element-wise operation:
% \begin{align}\label{eq:MLP}
%     \mathsf{MLP}(\Hb,\mathbf{\theta_2}) = \Wb_1 \mathsf{ReLU}(\Wb_2 \mathsf{Attn}(\Hb,\mathbf{\theta_1})),
% \end{align}
% where $\theta_2=\{\Wb_1,\Wb_2\}$ denotes the parameters of MLP. We remark that here some modules, such as layernorm and bias, are ignored for simplicity. 
% Note that the model parameters number is independent of the number of attention heads $h$, as each head projects the sequence into a $\frac{d_{\mathsf{hid}}}{h}$ subspace and then processes them.

\paragraph{Linear Attention-only Transformers} 
To perform an intractable theoretical investigation on the role of multi-head in the attention layer, we make simplifications on the transformer model by considering linear attention-only transformers. These simplifications are widely adopted in many recent works to study the behavior of transformer models \cite{vonoswaldTransformersLearnIncontext2023,zhang2023trained,mahankaliOneStepGradient2023,ahnTransformersLearnImplement,wu2023many}. In particular, the $i$-th layer $\mathsf{TF}_i$ performs the following update on the input sequence (or hidden state) $\Hb^{(i-1)}$ as follows:
\begin{equation}\label{eq:lsa_mha}
\begin{aligned}
    \Hb^{(i)} &= \mathsf{TF}_i(\Hb^{(i-1)}) \\
    &= \Wb_1 \big(\Hb^{(i-1)} + \mathsf{Concat}[\{\Vb_i \Mb \Kb_i^\top  \Qb_i \}_{i=1}^h]\big), \\
    \Mb&:= \begin{NiceArray}{\left\lgroup cc \right\rgroup}
\Ib_{n}& \mathbf{0}\\
\mathbf{0} & \mathbf{0}
\end{NiceArray} \in \RR^{m \times m},
\end{aligned}
\end{equation}
where $\{\Wb_{V_i}, \Wb_{K_i}, \Wb_{Q_i} \in \RR^{\frac{d_{\mathsf{hid}}}{h} \times d_{\mathsf{hid}}}\}_{i=1}^{h}$ and $\Wb_1  \in \RR^{d_{\mathsf{hid}} \times d_{\mathsf{hid}}}$ are learnable parameters. Besides, the mask matrix $\Mb$ is included in the attention to constrain the model focus the first $n$ in-context examples rather than the subsequent $m-n$ queries \cite{ahnTransformersLearnImplement,mahankaliOneStepGradient2023}. To adapt the transformer for solving sparse linear regression problems, we introduce additional linear layers $\Wb_E \in \mathbb{R}^{(d+1) \times d_{\mathsf{hid}}}$ and $\Wb_{O} \in \mathbb{R}^{d_{\mathsf{hid}} \times 1}$ for input embedding and output projection, respectively. Mathematically, let $\Eb$ denotes the input sequences with $n$ in-context example followed by $q$ queries, 
% where $\{\Wb_{V_i}, \Wb_{K_i}, \Wb_{Q_i} \in \RR^{\frac{d_{\mathsf{hid}}}{h} \times d_{\mathsf{hid}}}\}_{i=1}^{h}$ and $\Wb_1  \in \RR^{d_{\mathsf{hid}} \times d_{\mathsf{hid}}}$ are learnable parameters, note that as we ignore the $\mathsf{ReLU}$ activation in \Eqref{eq:MLP}, so we merge the parameter $\Wb_1 $ and $\Wb_2$ into one matrix $\Wb_1$. Besides, the mask matrix $\Mb$ is included in the attention to constrain the model focus the first $n$ in-context examples rather than the subsequent $m-n$ queries \cite{ahnTransformersLearnImplement,mahankaliOneStepGradient2023}. To adapt the transformer for solving sparse linear regression problems, we introduce additional linear layers $\Wb_E \in \mathbb{R}^{(d+1) \times d_{\mathsf{hid}}}$ and $\Wb_{O} \in \mathbb{R}^{d_{\mathsf{hid}} \times 1}$ for input embedding and output projection, respectively. Mathematically, let $\Eb$ denotes the input sequences with $n$ in-context example followed by $q$ queries, 
\begin{align}\label{eq:tf_input}
\Eb = \begin{NiceArray}{\left\lgroup ccccccc \right\rgroup}
\xb_1 & \xb_2 & \cdots & \xb_{n}& \xb_{n+1}&\cdots &\xb_{n+q}\\
y_1 & y_2 & \cdots & y_{n}& 0&\cdots &0\\
\end{NiceArray}.
\end{align}
Then model processes the input sequence $\Eb$, resulting in the output $\hat{\yb} \in \RR^{1 \times (n+q)}$:
\begin{align*}
\hat{\yb} = \Wb_{O} \circ \mathsf{TF}_L \circ \cdots \circ \mathsf{TF}_1 \circ \Wb_{E} (\Eb),
\end{align*}

here, $L$ is the layer number of the transformer, and $\hat{y}_{i+n}$ is the prediction value for the query $\xb_{i+n}$. During training, we set $q > 1$ for efficiency, and for inference and theoretical analysis, we set $q = 1$ and define the in-context learning excess risk $\mathcal{E}_{\mathsf{ICL}}$ as:
\begin{align*}
\mathcal{E}_{\mathsf{ICL}} := \EE_{(\xb,y)\sim \mathsf{P}} (\hat{y}_{n+1} - y_{n+1})^2 - \sigma^2.
\end{align*}

% \section{A Possible Mechanism}\label{sec: Mechanism}
% Based on observations from our experiments on performing sparse linear regression with transformers, we found that each head in the first layer of the trained transformer is crucial, while in subsequent layers, only one head plays a significant role. Therefore, we hypothesize that the trained transformer implements data preprocessing in the first layer, whereas subsequent layers perform gradient descent on the least squares loss function. Next, we propose a date pre-processing algorithm which the trained transformer is likely to implement.


% \begin{algorithm*}[t]
% \caption{\DPPSlR}\label{alg:DPPSLR}
% \small
% \begin{algorithmic}[1]
%   \STATE \textbf{Input :} Data set $\set{(\xb_i,y_i)}_{i=1}^n$.
  
  
%   \FOR{k=1,\ldots, n} 
%   \STATE Compute $\tilde{\xb}_k$ by $\tilde{\xb}_k=\Rh\xb_k$, where 
% $\Rh=\mathsf{diag}\set{\hat{r}_1, \hat{r}_2, \ldots, \hat{r}_d}$,
%   where $\hat{r}_j$ is  given by
%   \begin{align}
%       \hat{r}_j=\frac{1}{n}\sum_{i=1}^n \xb_{ij}y_i,
%   \end{align}
%   where $\xb_{ij}$ is the $j$-th entry of $\xb_i$.
%   \ENDFOR
% \STATE \textbf{Output :} Data set $\set{\paren{\tilde{\xb}_i,y_i}}_{i=1}^n$
% \end{algorithmic}
% \end{algorithm*}
% \paragraph{Intuition for Algorithm~\ref{alg:DPPSLR}} ...




==> icml_sections/related-work.tex <==
% \vspace{-.5em}
\section{Additional Related Work}

In addition to works towards understanding the expressive power of transformers that we introduced before, there is also a body of research on the mechanism interpretation and the training dynamics of transformers:

\paragraph{Mechanism interpretation of trained transformers} To understand the mechanisms in trained transformers, researchers have developed various techniques, including interpreting transformers into programming languages \cite{friedmanLearningTransformerPrograms, lindnerTracrCompiledTransformers2023a, weissThinkingTransformers2021,zhou2024what}, probing the behavior of individual layers \cite{pandit2021probing, wu2020perturbed, bricken2023towards,allen2023physics,zhu2023physics}, and incorporating transformers with other large language models to interpret individual neurons \cite{bills2023language}. While these techniques provide high-level insights into transformer mechanism understanding, providing a clear algorithms behind the trained transformers is still very challenging.

\paragraph{Training dynamics of transformers} In parallel, a body of work has also investigated how transformers learn these algorithms, i.e., the training dynamics of transformers. \cite{tarzanaghTransformersSupportVector2023} shows an equivalence between a single attention layer and a support vector machine. \cite{zhang2023trained,huang2023context} analyze the training dynamics of a single-head attention layer for in-context linear regression, where \cite{zhang2023trained} demonstrates that it can converge to implement one-step gradient over in-context examples. Additionally, \cite{tianScanSnapUnderstanding2023, li2023transformers} study the convergence of transformers on sequences of discrete tokens. These works provide valuable insights towards the theoretical understanding of the training dynamics of transformers, which offer potential future extension aspects for our work.

==> icml_sections/theory.tex <==
\vspace{-0.05in}
\section{Excess Risk of the Preprocess-then-optimize Algorithm}
\vspace{-0.05in}

\begin{figure*}[!t]
\vspace{-.1in}
\begin{minipage}{.225\textwidth}
\begin{subfigure}{\textwidth}
\includegraphics[width=\textwidth]{pic/preprocess_new.pdf}
\subcaption{P-probing}\label{fig:exp_fig1}
\end{subfigure}
\end{minipage}
\hfill
\begin{minipage}{.775\textwidth}
\begin{subfigure}{\textwidth}
\includegraphics[width=\textwidth]{pic/exp/preprocess/pre_gd_tf_1024.pdf}
\subcaption{P-Probing result for Transformers trained on varying heads and data settings}\label{fig:exp_fig2}
\end{subfigure}
\begin{subfigure}{\textwidth}
\includegraphics[width=\textwidth]{pic/exp/preprocess/pre_gd_new.pdf}
\subcaption{Directly apply Alg.~\ref{alg:DPPSLR} on input data for gradient descent}\label{fig:exp_fig3}
\end{subfigure}
\end{minipage}
\vskip -.1in
\caption{Supporting experiments for our preprocess-then-optimize algorithm and theoretical analysis}
\end{figure*}


In this section, we will develop the theory to demonstrate the improved performance of the preprocess-then-optimize algorithm compared to the gradient descent algorithm on the raw inputs. Appendix~\ref{sec:notation} provides a more detailed analysis.

% The proof for Theorem~\ref{thm: main}, \ref{thm:original_GD_general}, and \ref{thm:identitycase} can be found in Appendix~\ref{sec: proo_main}, \ref{sec:original_GD_general}, and \ref{sec:identitycase}, respectively.

We first denote $\twgd^t$ as the estimator obtained by $t$-step GD on $\set{\paren{\xt_i,y_i}}_{i=1}^n$, which can be viewed as the solution generated by the $t+1$-layer transformer based on our discussion in Section \ref{sec:Mechanism}, and $\wgd^t$ as the estimator obtained by $t$-step GD on $\set{(\xb_i,y_i)}_{i=1}^n$.
Before presenting our main theorem, we first need to redefine the excess risk of GD on $\set{\paren{\xt_i,y_i}}_{i=1}^n$. Note that in our algorithm, the learned predictor takes the form $\xb \to \langle \Rh \xb, \twgd^t \rangle$. Consequently, the population risk of a parameter $\twgd^t$ is naturally defined as $\tilde{L}(\twgd^t) \defeq \frac{1}{2} \cdot\mathbb{E}_{(\xb,y) \sim \mathsf{P}} \big[(\langle \Rh \xb, \twgd^t \rangle - y )^2 \big]$, and the excess risk is then defined as $\mathcal{E}(\wb) \defeq \tilde{L}(\wb) - \min_{\wb} \tilde{L}(\wb)$ \footnote{Here for the ease to presentation and comparison, we slightly abuse the notation of $\mathcal E(\wb)$ by extending it to $\twgd^t$, although $\mathcal E(\wb)$ is originally defined for the estimator for the raw feature vector $\xb$.}. 

% Next, we provide the upper bound of the excess risk for $\cE(\twgd^t)$ and $\cE(\wgd^t)$ respectively.
% \begin{theorem}\label{thm: main}
% Denote $\cS:=\{i:w^\star_i\neq 0\}$ and $\Rb=\mathsf{diag}\set{r_1,\ldots, r_d}$, where ${r_j}=\sum_{i=1}^d w^\star_i\Sigma_{ij}$. Suppose that there exist a $\beta>0$ such that $\min_{i\in\cS}\abs{r_i}\geq \beta$, $\normm{\Rb}_2,\normm{\Sigmab}_2, \normm{\ws}_2\simeq O\paren{1}$ and $n\gtrsim 1/\beta^2\cdot t^2s \cdot\big(\tr^{2/3}\paren{\Sigmab}+\tr\paren{\Rb\Sigmab\Rb}\big)\cdot\mathrm{poly}\paren{\log\paren{d/\delta}}$. Then set $\eta\lesssim 1/\normm{\Rb\Sigmab\Rb}_2$ and $
% \eta t\simeq \frac{1}{\beta}\cdot \big({\frac{\sigma^2\tr\paren{\Rb\Sigmab\Rb}\log\paren{d/\delta}}{n}+\frac{\sigma^2s\tr\paren{\Sigmab}\log^2\paren{d/\delta}}{n^2}}\big)^{-1/2}$, it holds that
% \begin{align*}
% \cE\paren{\twgd^t}
%     &\lesssim \frac{\log t}{\beta}\sqrt{{\frac{\sigma^2\tr\paren{\Rb\Sigmab\Rb}\log\paren{d/\delta}}{n}+\frac{\sigma^2s\tr\paren{\Sigmab}\log^2\paren{d/\delta}}{n^2}}},
% \end{align*}
% \whp.
% \end{theorem}
% Theorem \ref{thm: main} provides an upper bound on the excess risk achieved by the preprocess-then-optimize algorithm, where we tuned learning rate $\eta$ to balance the bias and variance error. Then, it can be seen that the risk bound is valid if $\tr\paren{\Rb\Sigmab\Rb}/n\rightarrow 0$ and $\tr(\bSigma) s/n^2\rightarrow 0$ when $n\rightarrow \infty$. This can be readily satisfied if we have $\|\wb^*\|_2$ and $\tr(\bSigma)$ be bounded by some reasonable quantities that are independent of the sample size $n$, which are the common assumptions made in many prior works \citep{zou2022risk,zou2021benefits,bartlett2020benign}. Besides, it can be also seen that the excess risk bound explicitly depends on the sparsity parameter $s$ and lower sparsity implies better performance. This implies the ability of the proposed preprocess-then-optimize for discovering and leveraging the nice sparse structure of the ground truth. 





% Furthermore, assume $w^\star_i\sim \mathsf{U}\paren{-1/\sqrt{s}, 1/\sqrt{s}}$ has a restricted uniform prior and $\min_{i\in\cS}\bSigma_{ii}\ge 1/\kappa$ for some constant $\kappa >1$, we can obtain that $\tr(\Rb\bsigma\Rb)\le \sum_{i\in\cS}\bSigma_{ii}/s$ and  $\beta \ge \sqrt{1/(s\kappa^2)}$. Ignoring $\sigma^2$ that appears in both $\cE\paren{\tilde \wgd^t}$ and $\cE\paren{\wgd^t}$, we have $\cE\paren{\tilde \wgd^t}\lesssim \tilde O(\sqrt{\kappa^2\sum_{i\in\cS}\bSigma_{ii}}{n}+\frac{s^2\kappa^2}{n})$.



% let $\cS$ be the set of feature indices that $w_i\neq 0$, we consider the case where $ \EE[x_ix_j] = 0$ for all $i \in \cS$ and all $j \notin \cS$ and $w^\star_i\sim \mathsf{N}\paren{\zero, 1/\sqrt{s}}$ for $i\in S$, which satisfies $\|\wb^*\|_2\eqsim\Theta(1)$ and $1/\beta=\cO\paren{\mathrm{poly}\paren{s}}$ with high probability. 







% Consequently, $\mathrm{tr}(\Rb \Sigmab \Rb) = \sum_{i \in S} r_i^2 \Sigma_{ii} \leq \mathcal{O}(s)$ (here we assume $|\Rb|_2, |\Sigmab|_2 = \Theta(1)$), which implies $\tilde{\mathcal{E}}(\twgd^t) \lesssim \mathrm{poly}(s)\cdot\sqrt{\frac{\sigma^2 }{n}+\frac{\tr\paren{d}}{n^2}}$, whereas $\cE\paren{\wgd^t}\lesssim \sqrt{\frac{\sigma^2\tr\paren{\Sigmab}}{n}}$ However, $\mathrm{tr}(\Sigmab)$ is $\mathrm{poly}(d)$ and much lager than $s$ in many cases; for example, when $\Sigmab = \Ib$, $\mathrm{tr}(\Sigmab) = d>>s$. Therefore, in this case, $\cE\paren{\wgd^t}\lesssim \mathrm{poly}(s)\cdot\sqrt{\frac{\sigma^2\tr\paren{\Sigmab}}{n^2}}<\sqrt{\frac{\sigma^2\tr\paren{\Sigmab}}{n}}$.


To make a formal comparison between preprocess-then-optimize and baselines, we consider the example where $x_i\iid \mathsf{N}\paren{\zerob,\Ib}$, based on which we can get the upper bound for our algorithm and the lower bound for OLS, ridge regression, and finite-step GD. 
\begin{theorem}\label{thm:identitycase}
Suppose $\cS$ with $\abs{\cS}=s$ is selected such that each element is chosen with equal probability from the set $\set{1,2,\ldots,d}$ and $w^\star_i\sim \mathsf{U}\{-1/\sqrt{s}, 1/\sqrt{s}\}$ has a restricted uniform prior for $i\in\cS$, $ \normm{\ws}_2\simeq \Theta\paren{1}$ and $n\gtrsim t^2s^3d^{2/3}$. Then there exists a choice of $\eta$ and $t$ such that
\begin{align*}
{\cE}\paren{\twgd^t}\lesssim 
   \sigma^2{\log^2\paren{ns/\sigma^2}\log^2\paren{d/\delta}}\cdot\paren{\frac{s}{n}+\frac{ds^2}{n^2}},
\end{align*}
\whp. Besides, let $\wla$ be the ridge regression estimator with regularized parameter $\lambda$, and $\wols$ be the OLS estimator, it holds that
\begin{align*}
&\EE_{\ws}\brac{\cE\paren{\wb}}\gtrsim 
    \begin{cases}
        {\frac{\sigma^2d}{n}}&n\gtrsim d+\log\paren{1/\delta}\\
       1-\frac{n}{d}+{\frac{\sigma^2n}{d}}&d\gtrsim n+\log\paren{1/\delta}, 
    \end{cases}
\end{align*}
\whp, where $\wb\in\{\wla,\wols,\wgd^t\}$.
\end{theorem}
It can be seen that for a wide range of under-parameterized and over-parameterized cases, $\twgd^t$ has a smaller excess risk than ridge regression, standard gradient descent, and OLS, when the sparsity $s$ satisfies $s=o\min\{d,n\}$. This justifies the effectiveness of the preprocess-then-optimize algorithm for dealing with the sparse regression problem. Moreover, it is well known that Lasso can achieve $\tilde O(s/n)$ excess risk bound in the setting of Theorem \ref{thm:identitycase}. Then we can conclude that the proprocess-then-optimize algorithm can be comparable to Lasso up to logarithmic factors when $d\lesssim n$, while becomes worse when $d\gtrsim n$.



% In particular, consider the setting $\sigma^2=1$, in the over-parameterized setting that $d\gtrsim n$, the excess risk bound of preprocess-then-optimize is $\tilde O(ds/n^2)$, which also outperforms the $\tilde \Omega(1)$ bound achieved by OLS, ridge regression, and standard gradient descent if the sparsity satisfies $s=O(n^2/d)$ (in fact, this condition can be certainly removed as ${\cE}(\twgd^t)$ also has a naive upper bound $\tilde O(1)$).  In the under-parameterized case that $d\lesssim n$, it can be readily verified that the data preprocessing can lead to a $\tilde O(s/n)$ excess risk, which is strictly better than the $\tilde \Omega(d/n)$ risk achieved by OLS, ridge regression, and standard gradient descent. Moreover, it is well known that Lasso can achieve $\tilde O(s/n)$ excess risk bound in the setting of Theorem \ref{thm:identitycase}. Then, by comparing with our results, we can also conclude that the proprocess-then-optimize algorithm can be comparable to Lasso up to logarithmic factors when $d\lesssim n$, while becomes worse when $d\gtrsim n$.




% \paragraph{Comparison with existing algorithms}Suppose that $s<<d$ and $1/\beta=\mathrm{poly}\paren{s}$. 
% When $n>d$, the excess risk of $\wla$, $\wols$ and $\wgd^t$ is lowered bound by ${\frac{\sigma^2d}{n}}$ which much lager than $\mathrm{poly}\paren{s}\cdot{\frac{\sigma^2}{n}+\frac{d}{n^2}}$. When $d^{2/3}<n<d$, the lower bound of $\cE\paren{\wla}$, $\cE\paren{\wols}$, $\cE\paren{\wgd^t}$ is lowered bound by $\cO\paren{\frac{\sigma^2n}{d}}$ which is also larger than the upper bound of $\tilde{\cE}\paren{\wpre_t}$, $\mathrm{poly}\paren{s}\cdot{\frac{\sigma^2}{n}+\frac{d}{n^2}}$. Therefore, when $\Sigmab=\Ib$, our algorithm performs strictly better than ridge regression, OLS, and GD. 
%  It is well-known that Lasso achieves
%  $\cO\paren{\frac{s}{n}}$ (here we hide the logarithmic terms). Our algorithm. Therefore, the upper bound of the excess risk for our algorithm is slightly worse compared to Lasso.
%  When $n>d$, $\tilde{\twgd^t}\lesssim \frac{\poly\paren{s}}{n}$, hence, the performance of our algorithm approaches that of Lasso in the case where $s$ is small. when $d^{2/3}<n<d$, the performance of our algorithm is worse than that of Lasso.


==> neurips2024/notations.tex <==
\def \parab{\overline{\para}}
\def \parab{\overline{\para}}
\newcommand{\rew}{\mathcal{R}^{\msf{all}}}
\newcommand{\rewfb}{\mathcal{R}^{\msf{feas}}_{[-B,B]}}
\newcommand{\rewfone}{\mathcal{R}^{\msf{feas}}_{[-1,1]}}
\newcommand{\rewfth}{\mathcal{R}^{\msf{feas}}_{[-3H,3H]}}

\newcommand{\tO}{\widetilde{\cO}}

\def \Vf{V^{\pp,r}}
\def \Qf{Q^{\pp,r}}
\def \piE{\pi^{\msf{E}}}
\def \hatpiE{\hat{\pi}^{\msf{E}}}
\def \pA{\overline{\cA}}
\def \pV{\overline{\cV}}
\def \para{\Theta}
% \def \rewm{\mathscr{R}}
% \def \RR{\rewm}
\def \fedb{e}
\def \wellpi{\Delta}
\def \wellsupp{n^{\msf{E}}}
\def \valsupp{n^{\msf{val}}}
\newcommand{\dpi}{d^\pi}
\newcommand{\dpiTheta}{d^\pi}
\newcommand{\DpiTheta}{D^\pi_\para}
\newcommand{\dall}{d^{\sf all}}
\newcommand{\dallTheta}{d^{{\sf all}}}
\newcommand{\DallTheta}{D^{\sf all}_\Theta}
\def \cn{\log\mathcal{N}(\Theta; \eps/H)}
\def \cns{\log\mathcal{N}}
\def \dimt{\dim\paren{\para}}
\def \pib{\pi^{\msf{b}}}
% \def \pival{\pi^{\msf{val}}}
\def \pival{\pi^{\msf{eval}}}
\def \dpival{d^{\pival}}
\def \Dpivalt{D^{\pival}_\Theta}
\def \DpiEt{D^{\piE}_\Theta}
% \def \hRR{\widehat{\RR}}
% \def \sRR{\RR^\star}
\def \hpp{\widehat{\pp}}
\def \DH{D^{\msf{H}}}
\def \DM{D^{\msf{M}}}
\def \Pidet{\Pi^{\mrm{determ}}}
\def \dpip{d^{\pp,\pi}}
\def \wellp{\eta}
\def \dt{\mrm{dim}\paren{\Theta}}
\def \hsa{[H]\times \cS\times \cA}


% Norms for convenience, along with sizes
% \newcommand{\norm}[1]{\left\|{#1}\right\|} % A norm with 1 argument
\newcommand{\lone}[1]{\norm{#1}_1} % l1 norm
\newcommand{\ltwo}[1]{\norm{#1}_2} % l2 norm
\newcommand{\lop}[1]{\norm{#1}_{\mathrm{op}}}
\newcommand{\lops}[1]{\|{#1}\|_{\mathrm{op}}}
\newcommand{\linf}[1]{\norm{#1}_\infty} % l-infinity norm
\newcommand{\lzero}[1]{\norm{#1}_0} % l0 norm
\newcommand{\dnorm}[1]{\norm{#1}_*} % Dual norm
\newcommand{\lfro}[1]{\left\|{#1}\right\|_{\sf Fr}} % Frobenius norm
\newcommand{\lnuc}[1]{\left\|{#1}\right\|_*} % Nuclear norm
\newcommand{\matrixnorm}[1]{\left|\!\left|\!\left|{#1}
  \right|\!\right|\!\right|} % Matrix norm with three bars
% \newcommand{\opnorm}[1]{\norm{#1}_{\rm op}} % Operator norm with three bars
\newcommand{\normbigg}[1]{\bigg\|{#1}\bigg\|} % A norm with 1 argument and bigg
                                              % brackets.
\newcommand{\normbig}[1]{\big\|{#1}\big\|} % A norm with 1 argument and big
                                           % brackets.
\newcommand{\normBig}[1]{\Big\|{#1}\Big\|} % A norm with 1 argument and Big
                                           % brackets
\newcommand{\lonebigg}[1]{\normbigg{#1}_1} % l1 norm
\newcommand{\ltwobigg}[1]{\normbigg{#1}_2} % l2 norm
\newcommand{\ltwobig}[1]{\normbig{#1}_2} % l2 norm
\newcommand{\ltwoBig}[1]{\normBig{#1}_2} % l2 norm
\newcommand{\linfbigg}[1]{\normbigg{#1}_\infty} % l-infinity norm
\newcommand{\norms}[1]{\|{#1}\|} % A norm with 1 argument and normal (small)
                                 % brackets.
\newcommand{\matrixnorms}[1]{|\!|\!|{#1}|\!|\!|} % Small matrix norm
\newcommand{\matrixnormbigg}[1]{\bigg|\!\bigg|\!\bigg|{#1}\bigg|\!\bigg|\!\bigg|} % Small matrix norm
\newcommand{\lones}[1]{\norms{#1}_1} % l1 norm with small brackets
\newcommand{\ltwos}[1]{\norms{#1}_2} % l2 norm with small brackets
\newcommand{\ltwob}[1]{\big\|#1\big\|_2}
\newcommand{\linfs}[1]{\norms{#1}_\infty} % l-infinity norm with small brackets
\newcommand{\lzeros}[1]{\norms{#1}_0} % l0 norm with small brackets
\newcommand{\lambdamax}[1]{\lambda_{\max}({#1})}
\newcommand{\lambdamin}[1]{\lambda_{\min}({#1})}
\newcommand{\vmax}[1]{v_{\max}({#1})}
\newcommand{\vmin}[1]{v_{\min}({#1})}


% Copied from headers of main text 
\def \dis{{d}}
% \def \cblue{\color{blue}}
% \def \cblack{\color{black}}
\def \cblue{}
\def \cblack{}
\newcommand{\online}{}
\newcommand{\bsh}{\textbackslash}
\newcommand{\va}{\V\times\a}
\def \dtheta{\mathrm{dim}\paren{\Theta}}
\def \Ctran{C^{\msf{tran}}}
\def \wCtran{C^{\msf{wtran}}}



% {\bf notations}
% \begin{itemize}
%  \item $\cA,~\cS,~ H$.~\yub{$\cA$ collides with $\cA$ set. Also, shall we use $\real^\cS$ or $\real^S$?}
% \item $r=\set{r_h(s,a)}_{h\in [H]},$
% \item $\pi=\set{\pi_h(\cdot|s)}_{h\in[H]}$
% \item $V^\pi_h(s;r,\pp)$. When it's clear from context, use $V^\pi_h(s;r)$.
% \item $Q^{\pi}_h(s, a;r)$
% \item \MDPR{}: $\m$. IRL problem: $\paren{\m, \piE}$.
% \item $d^\pi_h(s) \defeq \p(s_h = s|\pi)$
% \item $d^\pi_h(s, a) \defeq\p(s_h = s, a_h = a|\pi)$
% \item $A^{\pi}_h(s,a)$
% \item $\m\cup r$
% \item \textbf{operator.} $\brac{\pp_h V_{h+1}}(s,a)$, $\brac{\v_h V_{h+1}}(s,a)$, $\widehat{\pp}_h$, $\widehat{\v}_h$
% \item \textbf{feasible reward set.} $\cR_{\m,\piE}$
% \item \textbf{parameter set:} $A\in \pA$, $V\in \pV$. $\theta=(A,V)\in \para$~\yub{to be changed}
% \item \textbf{reward mapping:} $\rewm$, $r^\theta=\rewm\paren{V,A}=\rewm\paren{\theta}$
% \item \textbf{Feadback.} $\fedb$.
% \item \textbf{well-posedness.} for $\supp$: $\wellsupp$, for $\piE_h(a|s)$: $\wellpi$.
% \item \textbf{dimension of parameter space:} $\dimt$
% \item  \textbf{behavior policy:} $\pib$, \textbf{evaluation policy:} $\pival$, $\dpival$
% \item \textbf{metric for rewards.} $\dallTheta$, $\dpiTheta$, $\dpival$.
% \item \textbf{metric for reward mappings.} $\DallTheta$, $\DpiTheta$, $\Dpivalt$.
% \item \textbf{set of rewards.} $\rew$.
% \item \textbf{ground truth reward mapping.} $\sRR$, \textbf{recovered reward mapping.} $\hRR$.
% \item \textbf{recovered dynamics.} $\hpp$.
% \item \textbf{Hausdorff metric.} $\DH$. Mapping-based metric: $\DM$.
% \item \textbf{optimal policy set.} $\Pi^\star_{\m\cup r}$
% \end{itemize}




\def \DPPSlR{\textsc{Data Pre-processing for Sparse Linear Regression}}
\def \P{\mathsf{P}}
\def \wt{{\hat{\wb}_t}}
\def \ws{{\wb^\star}}
\def \Sigmab{\mathbf{\Sigma}}
\def\Xt{\tilde{\Xb}}
\def \xt{\tilde{\xb}}
\def \Sigmah{\hat{\Sigmab}}
\def \Sigmal{\overline{\Sigmab}}
\def\epsb{\mathbf{\epsilon}}
\def \Sigmat{\tilde{\Sigmab}}
\def \Rh{\hat{\Rb}}
\def \zerob{\mathbf{0}}
\def \contt{\alpha}
\def \nn{\frac{1}{n}}
\def \nnn{\frac{1}{n^2}}
\def \EEE{\cE}
\def \cont{{\tilde{\alpha}}}
\def \At{\tilde{\Ab}}
\def \wts{\tilde{\wb}^\star}
\def \Rl{\overline{\Rb}}
\def \whp{with probability at least $1-\delta$}
\def \wla{\hat{\wb}_{\lambda}}
\def\XXb{\Xb\Xb^\top}
\def\wols{\wb_{\mathrm{ols}}}
\def \wpre{{\hat{\wb}}}
\def \wgd{\wb_{\mathsf{gd}}}
\def \twgd{\tilde{\wb}_{\mathsf{gd}}}
